Prediction-sharing During Training and Inference

Two firms are engaged in a competitive prediction task. Each firm has two sources of data -- labeled historical data and unlabeled inference-time data -- and uses the former to derive a prediction model, and the latter to make predictions on new instances. We study data-sharing contracts between the firms. The novelty of our study is to introduce and highlight the differences between contracts that share prediction models only, contracts to share inference-time predictions only, and contracts to share both. Our analysis proceeds on three levels. First, we develop a general Bayesian framework that facilitates our study. Second, we narrow our focus to two natural settings within this framework: (i) a setting in which the accuracy of each firm's prediction model is common knowledge, but the correlation between the respective models is unknown; and (ii) a setting in which two hypotheses exist regarding the optimal predictor, and one of the firms has a structural advantage in deducing it. Within these two settings we study optimal contract choice. More specifically, we find the individually rational and Pareto-optimal contracts for some notable cases, and describe specific settings where each of the different sharing contracts emerge as optimal. Finally, in the third level of our analysis we demonstrate the applicability of our concepts in a synthetic simulation using real loan data.

==> addendum.tex <==
\trainEqNoSecond*
 
  \begin{proof}
 
Since the agents are symmetric, we assume a symmetric equilibrium is being played.\footnote{We note that this assumption is not required, and the result carries over to when an asymmetric equilibrium is played.} The possible symmetric equilibria are: (i) always predict $1$, (ii) always predict $0$, or $A \rightarrow 1, a \rightarrow 1$ (and the rest $0$). %\yotam{Maybe needs some explaining why $B\rightarrow 1, b \rightarrow 1$ can not happen}

As we saw in the proof of Lemma~\ref{lem:symmetric_reward_train_eq_no}, for a counter-example for $train-sharing = no-sharing$ we need to find $\theta_1, \theta_2$ so that there is a different train-sharing equilibrium in each. As we saw in previous proofs, the equilibrium condition of Equation~\ref{eq:conditional_equilibrium_condition} takes the form of predicting $1$ if and only if the conditional utility for predicting $1$ given the signal is non-negative. The conditional utility of predicting $1$ given some signal is linear in $\theta$ and so is monotone (possibly decreasing or increasing). We can thus constrain our search for the different equilibria outcomes to have $\theta_1 = \theta_{min}$ and $\theta_2 = \theta_{max}$. Moreover, there is monotonicity w.r.t. the equilibria types: More permissive equilibria (that predict $1$ more) will appear when the correlation is lower. We conclude that it is enough to look for such $\alpha$ and $C_1$ so that the equilibrium at $\theta_1 = \theta_{min}$ is different than the equilibrium at $\theta_2 = \theta_{max}$ among the three symmetric equilibrium options. For this we can analyze two cases of parametric equations in $\alpha, C_1$, and %the Bernoulli distribution $w$ over the possible correlations (world models) $\theta_{min}, \theta_{max}$. Writing down the equations directly, we 
find that no such $\alpha, C_1$ exist. %\yotam{This is done in the Mathematica files...}
%\ronen{Should we point to location in Mathematica files?}

 This is not always true. The wrong assumption is that the equilibria are monotone. Actually, when $C_1 = \frac{29}{64}R_1, \alpha = \beta = \frac{87}{128}, \theta = \frac{203}{320}$, two equilibria are acceptable: Either always predicting yes, or predicting yes upon the strong signal. And predicting upon the strong signal has higher utility for both firms. 
 
 \end{proof}
